Challenges in Measuring Transport Parameters of Carbonate-based Electrolytes

Numerical simulations are a powerful tool for the development and improvement of Li-ion batteries. Modeling the mass transport of the involved electrolytic solutions requires precise determination of the corresponding electrolyte parameters. In this work, we attempt to measure the conductivity, the diffusion coefficient, the transference number and the thermodynamic factor for a system of 0.5$\,$M LiPF$_6$ dissolved in a blend of ethylene carbonate and ethyl methyl carbonate (EC:EMC, 3:7 weight) at 20$\,${\deg}C and 50$\,${\deg}C. Applying galvanostatic polarization experiments to symmetrical metal Li | electrolyte + separator | Li metal cells reveals, however, a potential response qualitatively deviating from theoretical expectations. Impeded diffusion processes indicate the presence of additional, undesired porous structures on the Li electrodes, preventing a reliable evaluation of the electrolyte parameters. To spectrally resolve the diffusive processes, we conduct very-low-frequency impedance spectroscopy. The impedance in fact exhibits multiple interfering diffusive features. In our measurements, an explicit identification of the impedance for the sole diffusion through the separator is however not feasible. Therefore, the authors doubt that polarizing experiments using Li metal electrodes yield accurate parameters for electrolytes.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
